What Truly Grounds a Concept? Evidence-Aligned Concept Bottleneck Model

Concept Bottleneck Models (CBMs) route classifications through human-readable concepts, enabling inspection of classifier decisions. Yet correct concept predictions can rely on co-occurring parts or context rather than the intended visual evidence. We introduce EA-CBM (Evidence-Aligned Concept Bottleneck Model), which averages one spatial evidence map per concept into the bottleneck used for classification. Region-filter matching and spatial concept grounding align these maps with annotated regions. Matched regional perturbations encourage larger response drops under target-region removal than under control-region removal, while limiting control-induced changes. Region annotations are used only during training; inference requires the image alone. Across six datasets with concept-region annotations, EA-CBM achieves the highest concept mAP and Concept Trustworthiness Score (CTS) among twelve CBM baselines, improving CTS over each dataset's strongest method by 8.6 to 42.2 percentage points. Classification accuracy remains competitive with concept-supervised CBMs. With concept labels and masks on only 5% of training images and class supervision elsewhere, EA-CBM surpasses every baseline in CTS on all six datasets with regions.

==> tables/baseline_response.tex <==
\begin{table}[!t]
% cv-table-style
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.3804}
\caption{\textbf{Concept response to region removal for CEM, ProtoCBM, PGCM, and EA-CBM} on the six datasets with concept regions (one run each), with the test pairs, removals, and controls of Table~\ref{tab:response}. Responses are ProtoCBM's concept logits and, for CEM and PGCM, the logits of their concept probabilities; drops are in units of each response's test-set standard deviation. Share: percentage of pairs whose target decrease exceeds their mean control decrease.}
\label{tab:baseline_response}
\vspace{-0.5em}
\resizebox{0.99\columnwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\rowcolor{tbhead} \textbf{Dataset} & \textbf{Measure} & \textbf{CEM} & \textbf{ProtoCBM} & \textbf{PGCM} & \textbf{EA-CBM} \\
\midrule
 & Target drop & 0.07 & 0.05 & 0.45 & 0.20 \\
 & Control drop & 0.04 & 0.02 & 0.03 & 0.01 \\
\multirow{-3}{*}{\textbf{PACO-LVIS}} & Share (\%) & 51.3 & 52.8 & 64.6 & 78.2 \\
\midrule
\rowcolor{tbzebra}  & Target drop & 0.09 & 0.07 & 0.57 & 0.65 \\
\rowcolor{tbzebra}  & Control drop & 0.06 & 0.01 & 0.03 & 0.06 \\
\rowcolor{tbzebra} \multirow{-3}{*}{\textbf{Pascal-Part}} & Share (\%) & 62.0 & 69.4 & 72.8 & 94.2 \\
\midrule
 & Target drop & 0.23 & 0.59 & 1.45 & 0.71 \\
 & Control drop & 0.12 & 0.01 & 0.02 & 0.01 \\
\multirow{-3}{*}{\textbf{MonuMAI}} & Share (\%) & 69.3 & 82.1 & 85.1 & 95.5 \\
\midrule
\rowcolor{tbzebra}  & Target drop & 0.68 & 0.70 & 1.62 & 1.08 \\
\rowcolor{tbzebra}  & Control drop & 0.08 & 0.03 & 0.02 & 0.02 \\
\rowcolor{tbzebra} \multirow{-3}{*}{\textbf{FunnyBirds}} & Share (\%) & 82.8 & 92.6 & 88.2 & 96.4 \\
\midrule
 & Target drop & 0.49 & 0.14 & 1.05 & 2.35 \\
 & Control drop & 0.28 & 0.02 & 0.05 & 0.21 \\
\multirow{-3}{*}{\textbf{CUB}} & Share (\%) & 67.7 & 60.2 & 83.7 & 96.1 \\
\midrule
\rowcolor{tbzebra}  & Target drop & 0.13 & 0.42 & 1.35 & 3.26 \\
\rowcolor{tbzebra}  & Control drop & 0.08 & 0.07 & 0.03 & 0.07 \\
\rowcolor{tbzebra} \multirow{-3}{*}{\textbf{CelebA}} & Share (\%) & 53.8 & 70.5 & 92.1 & 100.0 \\
\bottomrule
\end{tabular}}
\end{table}

